Survey on Tools and Techniques Detecting Microservice API Patterns

It is well recognized that design patterns improve system development and maintenance in many aspects. While we commonly recognize these patterns in monolithic systems, many patterns emerged for cloud computing, specifically microservices. Unfortunately, while various patterns have been proposed, available quality assessment tools often do not recognize many. This article performs a grey literature review to find and catalog available tools to detect microservice API patterns (MAP). It reasons about mechanisms that can be used to detect these patterns. Furthermore, the results indicate gaps and opportunities for improvements for quality assessment tools. Finally, the reader is provided with a route map to detection techniques that can be used to mine MAPs.

==> Sections/tablePatterns2.tex <==

\begin{table}[b!]
\footnotesize
\centering
\caption{The list of Microservice API patterns~\cite{Zimmerman}}
\label{tab:patterns3}
\begin{tabular}{@{\,}p{11em}@{\,}p{10.3em}@{\,}p{9.5em}@{\,}}
\textbf{Foundation}         & \textbf{Quality}           & \textbf{Structure}             \\
Frontend integration        & API Key                    & Atomic Parameter               \\
Backend integration         & Rate Limit                 & Atomic Parameter List          \\
Public API                  & Rate Plan                  & Parameter Tree                 \\
Community API               & Service Level Agreement    & Parameter Forest               \\
Solution Internal API       & Error Report               & Data Element                   \\
API Description             & Conditional Request        & Id Element                     \\
\textbf{Responsibility}     & Request Bundle             & Link Element                   \\
Processing Resource         & Wish List                  & Metadata Element               \\
Information Holder Resource & Wish Template              & Annotated Parameter Collection \\
Computation Function        & Embedded Entity            & Context Representation         \\
State Creation Operation    & \textbf{Evolution}         & Pagination                     \\
Retrieval Operation         & Version Identifier         & \textbf{}                      \\
State Transition Operation  & Semantic Versioning        &                                \\
Operational Data Holder     & Two In Production          &                                \\
Master Data Holder          & Aggressive Obsolescence    &                                \\
Reference Data Holder       & Experimental Preview       &                                \\
Data Transfer Resource      & Limited Lifetime Guarantee &                                \\
Link Lookup Resource        & Eternal Lifetime Guarantee &                        
\end{tabular}

\end{table}

==> Sections/tableRQ1OSS.tex <==
\begin{table}[]
\scriptsize
\caption{OSS tools to detect Microservice Patterns (RQ1)}
\label{tab:rq1oss}
\centering
\begin{tabular}{lllll}

\textbf{Tool}              & \textbf{URL}   & \textbf{License} & \textbf{Lang. supported} & \textbf{Updated} \\ \hline
API security tools audit   & bit.ly/3GkQ38A & N/A (Free)       & REST API                 & N/A (Active)    \\
apidiff                    & bit.ly/3J0FyZN & MIT              & Java                     & 31.10.2021       \\
Arjun                      & bit.ly/3uFZoWv & GPL-3.0          & REST API                 & 29.08.2021       \\
Astra                      & bit.ly/3ontBp4 & Apache-2.0       & REST API                 & 05.04.2019       \\
Brakeman                   & bit.ly/3LbQtSo & MIT              & Ruby                     & 30.01.2022       \\
Coala                      & bit.ly/3AXgKiw & AGPL-3.0         & Any                      & 11.06.2021       \\
code2flow                  & bit.ly/34w2MYM & MIT              & Many (4)                 & 27.12.2021       \\
git-secret                 & git-secret.io  & MIT              & git                      & 01.02.2022       \\
git-semv                   & bit.ly/34yi1jM & MIT              & git                      & 17.06.2021       \\
GitVersion                 & bit.ly/3AVeUi6 & MIT              & git                      & 31.01.2022       \\
go-semrel-gitlab           & bit.ly/3upDINT & MIT              & git                      & 27.10.2019       \\
GraphQL FBC-CLI            & bit.ly/3orGVsz & OSS              & GraphQL                  & 06.06.2018       \\
Hikaku                     & bit.ly/3Hubkhx & Apache-2.0      & REST-API                 & 19.08.2021       \\
jgitver                    & bit.ly/3glahV5 & Apache-2.0       & Java                     & 30.03.2021       \\
Kiterunner                 & bit.ly/3J77eML & AGPL-3.0         & REST API                 & 10.05.2021       \\
LAPD                       & bit.ly/3gl6FlZ & N/A (Free)       & Java                     & 07.09.2013       \\
magento-semver             & bit.ly/3gnWygi & OSL-3.0          & N/A                      & 19.01.2022       \\
microservices-antipatterns & bit.ly/3GwBwGJ & Apache-2.0       & Python                   & 17.12.2019       \\
modver                     & bit.ly/32WbY8k & MIT              & Go                       & 16.01.2022       \\
Mondrian                   & bit.ly/3rqHkNZ & OSS              & PHP                      & 16.09.2014       \\
MSA-nose                   & bit.ly/3sgODXF & OSS              & Java                     & 12.04.2021       \\
next-ver                   & bit.ly/3B5EWzq & MIT              & git                      & 09.02.2018       \\
NodeJS scan                & bit.ly/3uqxHkm & GPL-3.0          & Node.js                  & 31.01.2022       \\
NoRegrets                  & bit.ly/3JjDAnF & Apache-2.0       & JavaScript               & 02.07.2019       \\
OpenAPI diff               & bit.ly/3oncymY & MIT              & REST API                 & 29.08.2017       \\
OpenAPI spec validator     & bit.ly/3AYY4yX & Apache-2.0       & REST API                 & 28.01.2022       \\
openapi-lint               & bit.ly/3oqUJDA & BSD-3            & REST API                 & 12.08.2020       \\
openapilint                & bit.ly/3J45Lqs & MIT              & REST API                 & 13.05.2019       \\
oval                       & bit.ly/3J466te & MIT              & REST API                 & 26.09.2018       \\
pact                       & bit.ly/3gp77Q8 & MIT              & REST-API                 & 03.02.2022       \\
paramspider                & bit.ly/3sf6JZZ & GPL-3.0          & REST API                 & 12.09.2021       \\
Prometheus                 & prometheus.io  & Apache-2.0       & Many (5)                 & 02.02.2022       \\
prospector                 & bit.ly/3oo4Zg7 & GPL-2.0          & Python                   & 01.02.2022       \\
Public API changes         & bit.ly/3gjOKMF & Unlicense        & C\#                      & 05.11.2017       \\
pycallgraph                & bit.ly/3uqyZfc & GPL-2.0          & Python                   & 28.02.2018       \\
Pyramid OpenAPI3           & bit.ly/3uqbZg5 & MIT              & Python                   & 07.12.2021       \\
pyramid-swagger            & bit.ly/3sfLKqb & BSD-3            & Python                   & 30.03.2020       \\
Python Semantic Release    & bit.ly/3oo3uyg & MIT              & Python                   & 31.01.2022       \\
REST API Antip. Inspect.   & bit.ly/3GkLhrG & MIT              & REST API                 & 31.03.2021       \\
schaapi                    & bit.ly/3J3BcB7 & MIT              & Java                     & 11.02.2019       \\
secret-detection           & bit.ly/3rqsM0N & OSS              & Any                      & 03.08.2020       \\
semantic-release           & bit.ly/34fFSFi & MIT              & git                      & 18.01.2022       \\
semantic-versioning-anal.  & bit.ly/3HsvgBn & MIT              & .NET                     & 03.11.2021       \\
semver-config              & bit.ly/3GnLpGN & OSS              & git                      & 26.09.2019       \\
semverbot                  & bit.ly/3GteoZI & MPL-2.0          & git                      & 03.01.2022       \\
Speccy                     & bit.ly/3uknqGe & MIT              & REST API                 & 02.10.2019       \\
Spectral                   & bit.ly/3gnIeo3 & Apache-2.0       & REST API                 & 03.02.2022       \\
SpotBugs                   & bit.ly/3glbvQj & LGPL-2.1         & Java                     & 29.01.2022       \\
Standard Version           & bit.ly/3uqgx64 & ISC              & Node.js                  & 01.01.2022       \\
Vulture                    & bit.ly/3Gq9hd2 & MIT              & Python                   & 03.01.2022       \\
wFuzz                      & bit.ly/3opt5Hg & GPL-2.0          & REST API                 & 28.11.2020       \\
Zally                      & bit.ly/34lLHkq & MIT              & REST API                 & 14.01.2022      
\end{tabular}
\end{table}

==> Sections/tableRQ3.tex <==
\newcolumntype{R}[2]{%
    >{\adjustbox{angle=#1,lap=\width-(#2)}\bgroup}%
    l%
    <{\egroup}%
}


% \begin{tabular}{l|ccc|ccc}
%  Patterns & \multicolumn{3}{c|}{Static Analysis} & \multicolumn{3}{c}{Dynamic Analysis}     \\ 
%   \hline
% &
% \rotS{Property 1} &
% \rotS{Property 2} &
% \rotS{Property 3} &
% \rotS{Property 1} &
% \rotS{Property 2} &
% \rotS{Property 3} 
%     \\ \hline
%  \multicolumn{7}{c}{\textbf{Foundation}}                                                                                                 \\ 
%         \hline
%         Frontend integration           & \checkmark & \checkmark  &            & \checkmark & \checkmark      &            \\ 
% \end{tabular}









\begin{table}
    \scriptsize
    \centering
    \caption{Possible Techniques for detecting microservice patterns}
    \refstepcounter{table}
    \label{tab:rq3}
    \vspace{.2em}
    \begin{tabular}{l|c|ccc|cc} 
        % \hline
           & \textbf{RQ2}                 & \multicolumn{5}{c}{\textbf{RQ3}}    \\ \cline{3-7} 
        Patterns   &  Detected by tool (ID)                  & \multicolumn{3}{c|}{Static} & \multicolumn{2}{c}{Dynamic}     \\ 
           &                     & \multicolumn{3}{c|}{Analysis} & \multicolumn{2}{c}{Analysis}     \\ 
        \hline
        
        &&
\rotV{Call Graph} &
\rotV{Source Code} &
\rotV{Repository} &
\rotV{Event Log} &
\rotV{Application log} 
%\rotV{System log}
\\
        
        
              %                         & Call Graph & Source Code & Repository & Event Log  & Application log & System log \\ 
        \hline
        \multicolumn{7}{c}{\textbf{Foundation}}                                                                                                 \\ 
        \hline
        Frontend integration      &     & \checkmark & \checkmark  &            & \checkmark & \checkmark                 \\ 
        \hline
        Backend integration     &    & \checkmark & \checkmark  &            &            &                           \\ 
        \hline
        Public API          &           &            &             &            &            &                            \\ 
        \hline
        Community API                  &            &             &            &            &                 &            \\ 
        \hline
        Solution Internal API          &            &             &            &            &                 &            \\ 
        \hline
        API Description                &            &             &            &            &                 &            \\ 
        \hline
        \multicolumn{7}{c}{\textbf{Responsibility}}                                                                                             \\ 
        \hline
        Processing resource      &      & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Information holder resource  &  & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Computation function     &      & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        State recreation operation  &   & \checkmark & \checkmark  &            & \checkmark & \checkmark                 \\ 
        \hline
        Retrieval operation      &      & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        State transition operation  &   & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Operational Data Holder    &    & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Master data holder         &    & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Reference data holder &         & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Data transfer resource    &     & \checkmark & \checkmark  &            & \checkmark & \checkmark       \\ 
        \hline
        Link Lookup resource     &      & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        \multicolumn{7}{c}{\textbf{Structure}}                                                                                                  \\ 
        \hline
        Atomic parameter             &  &            & \checkmark  &            &            &                             \\ 
        \hline
        Atomic parameter list    &      &            & \checkmark  &            &            &                             \\ 
        \hline
        Parameter tree       &          &            & \checkmark  &            &            &                             \\ 
        \hline
        Parameter forest       &        &            & \checkmark  &            &            &                            \\ 
        \hline
        Data element       &            &            & \checkmark  &            &            &                             \\ 
        \hline
        Id element        &             &            & \checkmark  &            &            &                             \\ 
        \hline
        Link element         &          &            & \checkmark  &            &            &                             \\ 
        \hline
        Metadata element       &        &            & \checkmark  &            &            &                             \\ 
  %      \hline
   %     Annotated parameter collection &&           &            &           &           &                          \\ 
        \hline
        Context representation        & &            & \checkmark  &            &            &                             \\ 
        \hline
        Pagination               &      &            & \checkmark  &            & \checkmark & \checkmark                 \\ 
        \hline
        \multicolumn{7}{c}{\textbf{Quality}}                                                                                                    \\ 
        \hline
        API key             &           &            & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Rate limit        &             &            & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Rate plan           &           &            &             &            &            &                             \\ 
        \hline
        Service level agreement  &      &            &            &            &            &                             \\ 
        \hline
        Error report         &          & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Conditional request     &       & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Request bundle      &           & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Wish list           &           & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Wish template     &             & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Embedded entity      &          & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        Linked information holder   &   & \checkmark & \checkmark  &            & \checkmark & \checkmark                  \\ 
        \hline
        \multicolumn{7}{c}{\textbf{Evolution}}                                                                                                  \\ 
        \hline
        Version identifier         &    &            & \checkmark  & \checkmark & \checkmark &                             \\ 
        \hline
        Semantic versioning         &   &            & \checkmark  & \checkmark & \checkmark &                             \\ 
        \hline
        Two in production        &      &            & \checkmark  & \checkmark & \checkmark &                             \\ 
        \hline
        Aggresive obsolesense       &   & \checkmark & \checkmark  & \checkmark & \checkmark &                             \\ 
        \hline
        Experimental preview        &   &            & \checkmark  & \checkmark & \checkmark &                             \\ 
        \hline
        Limited lifetime guarantee   &  &            &             &            &            &                             \\ 
        \hline
        Eternal lifetime guarantee  &   &            &             &            &            &                             \\
        \hline
    \end{tabular}
    
\end{table}
